Driving Style Recognition Using Interval Type-2 Fuzzy Inference System and Multiple Experts Decision Making

Driving styles summarize different driving behaviors that reflect in the movements of the vehicles. These behaviors may indicate a tendency to perform riskier maneuvers, consume more fuel or energy, break traffic rules, or drive carefully. Therefore, this paper presents a driving style recognition using Interval Type-2 Fuzzy Inference System with Multiple Experts Decision-Making for classifying drivers into calm, moderate and aggressive. This system receives as input features longitudinal and lateral kinematic parameters of the vehicle motion. The type-2 fuzzy sets are more robust than type-1 fuzzy sets when handling noisy data, because their membership function are also fuzzy sets. In addition, a multiple experts approach can reduce the bias and imprecision while building the fuzzy rulebase, which stores the knowledge of the fuzzy system. The proposed approach was evaluated using descriptive statistics analysis, and compared with clustering algorithms and a type-1 fuzzy inference system. The results show the tendency to associate lower kinematic profiles for the driving styles classified with the type-2 fuzzy inference system when compared to other algorithms, which is in line with the more conservative approach adopted in the aggregation of the experts' opinions.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}



==> tex/old_related_works.tex <==
% As mentioned before, there are many applications for direction style recognition, so there is no standard for defining classes (e.g., calm and aggressive), as well as, different techniques can be applied. Due to the lack of a large and labeled database for driving styles, most of the literature uses either unsupervised machine learning techniques, statistical analysis, or rule-based methods. Table \ref{tab:related_works} shows some related works with the techniques applied and driving style classes.  


% In Johnson and Trivedi \cite{johnson2011driving} a driving maneuver detection with driving style distinction between `Non-Aggressive' and `Aggressive', for each maneuver, was developed using Dynamic Time Warping (DTW) and smartphone based sensor-fusion (accelerometer, gyroscope, magnetometer, GPS, and video), recording potentially-aggressive events. The disadvantages of the proposed method are the calibration of the smartphone sensors, including the positioning of the smartphone in the vehicle, and the sensitivity of the approach to noise from sensors, being minimized only by a low-pass filter.  In turn,   Han et al. \cite{han2018statistical} proposed a statistical-based driving style recognition, between `Normal' and `Aggressive', by modeling the driver behavior uncertainty with kernel density estimation, and classifying styles with a modified Bayesian Decision using Euclidean distance. They also developed a fuzzy inference system to compare the approaches. The disadvantages of this system are the scalability of the number of driving style classes, and the use of only longitudinal features (i.e., vehicle speed, throttle opening, and longitudinal acceleration) of the vehicle's movement. 


%  Xing, Lv, and Cao \cite{xing2019personalized} presented an intention-aware trajectory prediction based on driving style recognition, in which a Gaussian Mixture Model (GMM) Clustering classifies styles into `Conservative', `Moderate', and `Aggressive'. For each class, a specific MLP (Multi-layer Perceptron) perform  the regression of the predicted trajectory, using also the features extracted from a LSTM (Long Short-Term Memory). This approach was validated using the NGSIM dataset, which is known to have significant noise data with impossible kinematics parameters. To use these data, the authors used an interpolated curve method and a low-pass filter to reduce the effect of the noisy data. In  Qi et al. \cite{qi2015leveraging} an ensemble clustering method (ECM) based on the Kernel Fuzzy C-means (KFCM) and the modified Latent Dirichlet Allocation (LDA) was applied for driving style recognition by analyzing longitudinal features of the vehicle's kinematics (i.e., velocity and acceleration), and the time gap between the leader vehicle and the rear vehicle (target) in a car-following scenario. 


%  Suzdaleva and Nagy \cite{suzdaleva2018online} developed a  recursive Bayesian mixture-based cluster analysis for driving style recognition, which was applied in a fuel-saving application. The method identifies the level of fuel consumption, also taking into account velocity, gas pedal position, and gear. The recursiveness of the application occurs when the classification at the current time depends on the driving style detected at previous time stamp for the same vehicle. Constantinescu, Marinoiu and Vladoiu \cite{constantinescu2010driving} performed statistical analysis using Principal Component Analysis (PCA) and Hierarchical Cluster Analysis (HCA) for classifying drivers in driving styles that are more likely to commit traffic violations or get involved in accidents. The method analyzed data from 23 different drivers gathered within 2 to 5 working days, using statistical features of the kinematics parameters, such as mean and standard deviation of the speed, acceleration, positive acceleration, braking (negative acceleration), and mechanical work. The  time window of days allowed the authors to identify more time-consistent driving styles instead of transient styles, which are the objective of real-time applications.


% Similarly, Liu et al. \cite{liu2019research} applied PCA, Fuzzy C-Means (FCM) clustering, and Support Vector Machine (SVM), with data from 51 drivers, and classifies them into `Conservative', `General', and `Aggressive'. Each driver drove a 25Km route with an average time of $40$ min. The proposed approach analyzed longitudinal features of the routes (i.e., velocity, longitudinal acceleration, and gas pedal), after discretizing them with information entropy. PCA was used to reduce the dimension of the feature vector created using statistical features (i.e., mean and standard deviation) of the data.


% In addition to the aforementioned learning-based, model-based, and statistical methods for driving style recognition, there are also rule-based techniques that are able to represent experts knowledge using  rules,  such as \emph{\textbf{if} \underline{logical preposition} \textbf{then} \underline{logical consequence}}.  Murphey, Milton and Kiliaris \cite{murphey2009driver} presented a driving style classification based on the analysis of the jerk profile of the vehicle, which classifies segments of the route into `Calm', `Normal', and `Aggressive' styles. The algorithm calculates the ratio of the standard deviation of the jerk profile within a time window, and the mean of the jerk in a specific road-type (e.g., freeway and ramps). A threshold-based analysis is then used for classification. The authors compared the performance of the system with time windows of sizes 15, 9, 6, and 3 seconds, in which, 9 and 6 obtained the best results. The disadvantages of the method are the calibration of the thresholds, that must also be robust to noise; the use of only one feature to characterize a driving styles; the use of only longitudinal features; and, the difficulty of characterizing an average driving style for a specific road-type using only the mean of the jerk profile. 


% Besides threshold-based analysis, Fuzzy Inference Systems (FIS) are also used for driving style recognition.   Aljaafreh, Alshabatat and Al-Din \cite{aljaafreh2012driving} proposed a FIS for driving style classification using longitudinal features gathered from a 2-axis accelerometer, into `Below Normal', `Normal', `Aggressive', and `Very Aggressive' styles. The input of the system is the euclidean norm of the lateral and longitudinal acceleration, filtered by a moving average filter, and the velocity. Similarly,  Dörr, Grabengiesser and Gauterin \cite{dorr2014online} also employed a FIS for driving style recognition. Their system  extracted the input features from the CAN (Controller Area Network) bus of the vehicle, and a road class (e.g., dirt track, urban street, rural roads, and freeway) from the navigation system. Specifics FIS were developed for each road class, and each one also uses different set of input parameters (e.g. acceleration, velocity, deceleration, time gap). The authors also used a Kalman Filter to reduce noise in the data.


% This paper proposes a Fuzzy Inference System for driving style recognition, but, instead of use standard Type-1 Fuzzy Sets, we used Interval Type-2 Fuzzy Sets \cite{chen2013fuzzy}, which are more robust to uncertainty and subjectivity inherent to the rule-based logic system. In addition, the rules of the system were created using Fuzzy Multiple Experts Decision-Making, with type-1 fuzzy aggregation operator, known as OWA (Ordered Weighted Averaging), which also reduces the bias of experts in creating  the system's rules \cite{vanivcek2009fuzzy,chen2010fuzzy,zhou2008type}. The proposed system was validated with the publicity available large scale dataset Argoverse  \cite{chang2019argoverse}, and compared with clustering algorithms (i.e., K-Means, GMM clustering, Fuzzy C-means, and Agglomerative Hierarchical Clustering) using descriptive statistics analysis over the clusters or classes. The input  combines statistical features (i.e., mean and standard deviation) of longitudinal (i.e., velocity, acceleration, and deceleration) and lateral (i.e., lateral jerk) kinematics parameters of the vehicle's movement over a time window. All the input features are derivative of the space (position of the vehicle), therefore, for estimating their values and to reduce the noise, the proposed approach evaluates the use of Extended Kalman Filter (EKF) and SavitzkyGolay filter.    

==> tex/old_results.tex <==
% In order to evaluate the proposed T2-FIS, we used descriptive statistical analysis of the groups found as result of the classification, and compared them with four clustering algorithms, in addition to a T1-FIS build with only the upper membership function of the type-2 fuzzy sets, shown in Table \ref{tab:type2_fis:parameters}.  The data were obtained from the public dataset called Argoverse \cite{chang2019argoverse}.
% The implementations of the clustering algorithms, the type-1 and type-2 fuzzy systems, and the extraction and pre-processing of data, are available in a public repository on GitHub\footnote{\url{https://github.com/iag0g0mes/t2fis_driving_style.git}}. The following sections detail the dataset and the pre-processing step, the evaluation metrics and benchmark techniques, and the experimental results. 

% \subsection{Dataset}
% \label{subsec:results:datasets}

% The Argoverse dataset was developed by the North American company Argo AI, in partnership with Carnegie Mellon and Georgia Institute of Technology universities. The database has data from several sensors and semantic maps of the environment in several American cities. In addition, it offers support for 3D object tracking and path prediction tasks, containing information from more than ten thousand tracked objects, including trajectories at intersections, lane change, traffic jams and curves \cite{chang2019argoverse}.

% In this paper we use the motion forecasting dataset that has $324\;557$ scenarios, each $5$ seconds long, divided into sample, training, testing, and validation. We extracted the features (i.e., mean velocity, mean acceleration, mean deceleration, standard deviation of the lateral jerk) from the training and validation sets, with $205\;942$ and $39\;472$ samples, respectively. The window's size to measure the features was 5 seconds. The training data was used to build all models, and the validation data was used for evaluation. Table \ref{tab:dataset:val} shows the  descriptive statistical analysis of the validation data. 

% \input{tex/tab_dataset_val}

% All features were estimated through the derivative of the space, since the dataset only provides the position of the vehicles and the timestamp. Based on Table \ref{tab:dataset:val}, it is possible to highlight the large amount of noise when we estimate the features from the \emph{raw} data, resulting in unrealistic measures. Thereby, we applied two filters to reduce the noise, an Extended Kalman Filter (EKF) and SavitzkyGolay filter. The noise reduction from the SavitzkyGolay filtering was larger than the EKF, although this technique uses polynomial interpolation for smoothing the data, while the EKF uses dynamic equations of the vehicle motion in a cycle with prediction, using the equations, and correction, using the observations.    

% \subsection{Evaluation Metrics}
% \label{subsec:results:evaluation_metrics}


% There are some challenges in assessing driving style recognition without labeled data, since most of the evaluation metrics measure how well a method performs compared to the ground truth of the data. Some related works apply either supervised metrics (e.g., confusion matrix, accuracy, etc.) or clustering analysis with manually labeled data, obtained either in simulation \cite{han2018statistical,dorr2014online} or by some drivers who participated in the research \cite{johnson2011driving,suzdaleva2018online,constantinescu2010driving, liu2019research}. However, the amount of data, diversity of traffic situations, and the representativeness of kinematic profiles are more limited than public and large-scale datasets like Argoverse. In addition, studies with private data make it difficult for comparisons to be made with other studies in the literature. Some articles use private datasets to perform qualitative evaluations of the methods \cite{aljaafreh2012driving}, qualitative analysis of the results obtained \cite{qi2015leveraging,constantinescu2010driving}, or perform analysis of an external variable, such as fuel consumption, to interpret the results \cite{murphey2009driver,suzdaleva2018online}.

% According to  Greene, Cunningham and Mayer \cite{greene2008unsupervised}, in the absence of labeled data, there is no clear definition of what constitutes correct clustering. Therefore, it is possible to evaluate the result employing qualitative methods, and quantitative metrics through internal validation of the clusters, which measures how well-defined the clusters are, for instance, how much the clusters intersect and the variability of each group. Another way to evaluate the result is the descriptive statistical analysis which summarizes the data distribution with central tendency, and dispersion measures \cite{demaris2013summarizing}.



% Therefore, the proposed T2-FIS with multiple experts decision-making is evaluated using descriptive statistical analysis, using  mean as a measure of central tendency, standard deviation, minimum value, maximum value, and quantiles as measures of dispersion. The analysis of descriptive statistics allows understanding how behaves the data distribution in each driving style (e.g., \emph{calm}, \emph{moderate}, and \emph{aggressive}), being able, therefore, to indicate the tendencies of the kinematic parameters for each class. For instance, it is possible to know from the central tendencies of the parameters which drivers adopt more conservative and safer actions. The dispersion of data in each class, on the other hand, allows us to know the consistency of the data in relation to their central tendencies, in addition to the influence of noise on each class.




% Moreover, the proposed system is also compared with the implementation of four clustering algorithms \cite{xu2015comprehensive}, i.e., K-Means, Agglomerative Hierarchical Clustering, Fuzzy C-Means Clustering, and Gaussian Mixture Clustering, and also with a Type-1 Fuzzy Inference (T1-FIS) System built using the upper membership functions, shown in Table \ref{tab:type2_fis:parameters}. The experiments with the T1-FIS and T2-FIS were performed using both single and multiple experts approaches, in which the same single expert was used for both T1-FIS and T2-FIS.
 
 
 
% In addition to descriptive statistics, we also evaluated the clustering algorithms using three clustering analysis metrics  \cite{greene2008unsupervised}, namely:  Silhouette Coefficient, which estimates a value within the range $[-1,1]$, indicating how well allocated the data is in their respective clusters, with values close to $1$ being the best indicator; Calinski-Harabasz Score, in which a larger value indicates better-defined clusters with a large degree of clusters separation; and, Davis-Bouldin Index, where a lower value implies clustering algorithm with more compact and more distinctly separated clusters. 


% \subsection{Driving Style Recognition}
% \label{subsec:results:driving_style_recognition}

% In order to evaluate the proposed T2-FIS with multiple-experts decision-making, we compare its results with clustering algorithms and a T1-FIS using descriptive statistics analysis. According to  DeMaris and Selman \cite{demaris2013summarizing}, descriptive statistics summarizes the data distribution, which allow us to understand how each of the driving styles behaves regarding the tendency of the kinematics features. 

% Table \ref{tab:result:clustering:descriptive_stats} shows the results of the four clustering algorithms, i.e., K-Means, Gaussian Mixture Models (GMM) Clustering, Fuzzy C-Means, and, Agglomerative Hierarchical Clustering. The outputs of clustering algorithms are clusters parameters, such as centers of each cluster, and, the label of each cluster is assigned lastly from the analysis of an expert. From Table \ref{tab:result:clustering:descriptive_stats}, it is possible to highlight the conformity of each driving style with the expected kinematics profiles, that is, the \emph{calm} driving style has a lower profile than the \emph{moderate} style, which, in turn, is lower than the \emph{aggressive} style. 

% The central tendencies of the \emph{calm} driving style of all clustering algorithms are on average $(8.29, 3.93, 3.75, 36.49)$, using the data filtered by the EKF filter, and $(5.61, 1.44, 1.425, 1.27)$ with the data filtered with the SavitzkyGolay filter,  for the features `\emph{Mean Velocity}', `\emph{Mean Acceleration}', `\emph{Mean Deceleration}', and `\emph{STD Lateral Jerk}', respectively. In turn, the means of the kinematics parameters of the \emph{moderate} driving style are $(10.27, 7.59, 7.30, 92.31)$ with the EKF filter, and $(10.52, 0.93, 0.94, 1.20)$ with the SavitzkyGolay filter. Meanwhile, the \emph{aggressive} driving style has means equal to $(11.41, 13.26, 12.27, 185.78)$ and $(14.24, 1.49, 1.65, 2.15)$, using the EKF and SavitzkyGolay filters, respectively. 

% % \input{tex/tab_clustering}
% % \input{tex/tab_fuzzy}

% Table \ref{tab:clustering_analysis} shows the results of the internal clustering evaluation metrics of the four clustering algorithms. As stated in  Greene, Cunningham and Mayer \cite{greene2008unsupervised}, the closer the value of the \emph{Silhouette Coefficient} is to 1 the better allocated the data are to their respective clusters. Thus, from Table \ref{tab:clustering_analysis}, the algorithms that have the best silhouette coefficient are the \emph{Agglomerative Hierarchical Clustering} (EKF) and \emph{K-Means} (SavitzkyGolay). However,  \emph{K-Means} clustering outperforms the other clustering algorithms in the other two evaluation metrics, i.e., \emph{Calinski Harabasz Score} and \emph{Davis-Bouldin Index}. Another important conclusion shown in the Table \ref{tab:clustering_analysis} is the lower values obtained in the evaluation metrics for the data filtered with the SavitzkyGolay filter, which can be explained by the low spread of the data (see Table \ref{tab:dataset:val}), measured by the standard deviation, 
% which shows that the data are closer in the feature space, making the separation of clusters more difficult.

% \input{tex/tab_clustering_analysis}

% \input{tex/tab_centers_kmeans}

% The results of the fuzzy inference system, shown in Table \ref{tab:fuzzy_result}, are divided into two experiments for both the T1-FIS and the proposed T2-FIS, being \emph{single} with the rulebase built using a single expert, and \emph{multiple} with the rulebase built with aggregation of eight experts' opinions, $n=8$, (see sections \ref{subsec:fuzzy2:multiple_experts_dm} and \ref{subsec:method:fmedm}). 



% Taking into consideration only the experiments with a \emph{single} expert,  the central tendencies of the \emph{calm} driving style are on average $(4.70, 1.67, 1.61, 7.64)$ with the EKF filter, and $(8.5, 1.1, 1.09, 1.2)$ using the SavitzkyGolay filter. The \emph{moderate} driving style has means equal to $(7.60, 3.69, 3.43, 38.30)$ and $(14.45, 1.62, 1.79, 2.16)$, for, respectively, the EKF and SavitzkyGolay filters. In addition, the means of \emph{aggressive} driving style are  $(10.74, 8.01, 7.65, 95.5)$, using the EKF filter, and  $(17.31, 4.68, 5.1, 6.62)$, using the SavitzkyGolay filter.  


% Alternatively, the results using the \emph{multiple} experts approaches showed that, the central tendencies of the \emph{calm} driving style are on average $(3.53, 1.65, 1.57, 7.31)$ and  $(6.19, 1.16, 1.13, 1.14)$, using the EKF and SavitzkyGolay filter, respectively. In turn, the \emph{moderate} driving style has means equals to $(6.88, 2.89, 2.65, 28.00)$, and  $(12.64, 1.21, 1.3, 1.58)$, while the \emph{aggressive} driving style has means equals to $(10.18, 7.44, 7.1, 87.9)$, and $(17.6, 5.07, 5.06, 6.85)$, using, in this order, the EKF and SavitzkyGolay filter. 

% The central tendencies and standard deviations of the \emph{multiple} experts approaches are lower than the \emph{single} experts approaches for most of the features, in both the EKF and SavitzkyGolay filters.  These results show that the \emph{multiple} experts approaches find more distinct and regular kinematic profiles for each driving style, since spreads of the data from their central tendencies are lower.   

% Besides the difference in the means and standard deviations of the data for each driving style among the experts approaches, the data dispersion, measured by the quantiles, are also distinct. The quantiles $\mathcal{Q}_{0.75}$, also known as third quartile ($\mathrm{Q}_{3}$), which represents the upper limit of $75\%$ of the data, of the \emph{single} expert approaches, are on average for data filtered by EKF and SavitzkyGolay filters, respectively:  \emph{calm}, $(5.97, 2.08, 1.98, 9.5)$ and $(11.24, 1.53, 1.52, 1.6)$; \emph{moderate}, $(8.88, 4.65, 4.23, 49.19)$ and $(17.23, 2.21, 2.5, 3.03)$; and, \emph{aggressive}, $(14.23, 9.92, 9.49, 123.38)$ and $(19.55, 6.91, 6.22, 8.47)$. In turn, the quantiles $\mathcal{Q}_{0.75}$, of the \emph{multiple} expert approaches are, in the same order: \emph{calm}, $(4.21, 2.09, 1.94, 9.35)$ and $(7.96, 1.63, 1.58, 1.5)$; \emph{moderate}, $(8.88, 3.33, 3.08, 35.32)$  and $(14.98, 1.56, 1.74, 2.05)$; and, \emph{aggressive}, $(13.43, 9.17, 8.78, 112.99)$ and $(21.14, 7.19, 7.11, 8.98)$. 

% These quantile values also indicate the lower kinematic tendency of the \emph{multiple} experts approach compared to the \emph{single} expert approach. The only exception is the \emph{aggressive} style using the SavitzkyGolay filter, which occurred because some instances classified as \emph{aggressive} in the \emph{multiple} experts approach were classified as \emph{moderate} using only a \emph{single} specialist. These differences can be observed by the limits maximum and minimum values in Table \ref{tab:fuzzy_result}.

% The descriptive statistics analysis also show differences between the T1-FIS and the T2-FIS using \emph{multiple} experts approach. 
% The central tendencies of the features, `\emph{Mean Acceleration}' and `\emph{Mean Deceleration}', are lower in the T2-FIS than the T1-FIS, except for the \emph{moderate} and \emph{aggressive} driving styles using the data filtered with the SavitzkyGolay filter. Similarly, the maximum value for the two features in the results of the T2-FIS is less than or equal to the maximum values of the T1-FIS.

% In addition, the interquartile ranges (IQR) of the `\emph{STD Lateral Jerk}', which has the highest amount of noise, as shown in Table \ref{tab:dataset:val}, show that its variation for each driving style class is lower with the T2-FIS, being: $3.77$ (EKF) and $0.93$ (SavitzkyGolay), for the \emph{calm} driving style; $14.45$ (EKF) and $1.47$ (SavitzkyGolay), for the \emph{moderate} style; and, $64.43$ (EKF) and $4.40$ (SavitzkyGolay), for the \emph{aggressive} style. The IQR values of the T1-FIS for the \emph{calm}, \emph{moderate}, and \emph{aggressive}, are, in this order: $3.78$ (EKF) and $0.96$ (SavitzkyGolay); $17.97$ and $1.32$; and, $65.26$ and $6.01$. The only exception is the IQR of the \emph{moderate} driving style using SavitzkyGolay filter due to the difference of the quantiles $\mathcal{Q}_{0.75}$, which are $1.96$ (T1-FIS) and $2.14$ (T2-FIS).     


% The differences of the descriptive statistics between the clustering algorithm and the T2-FIS using \emph{multiple} experts approach are also notable in the analysis of Table \ref{tab:result:clustering:descriptive_stats} and Table \ref{tab:fuzzy_result}. The contrast can also be noticed by the euclidean distance between the centers of the clusters from the K-Means, shown in Table \ref{tab:centers_kmeans},  and the central tendency of the T2-FIS. These distances are, considering the order of the application of the EKF and SavitzkyGolay filters: \emph{calm}, $(28.08, 9.65, 49.89)$ and $(1.72, 7.77, 14.91)$; 


% These distances show that the center of the \emph{calm} cluster, using the EKF filter, is closer to the central tendency of the data classified as \emph{moderate} by the T2-FIS, while the center of the \emph{moderate} (K-Means) is closer to the central tendency of the \emph{aggressive} (T2-FIS). In turn, the center of the \emph{aggressive} style (K-Means), using the SavitzkyGolay filter, is closer to the \emph{moderate} style in the T2-FIS. Therefore, the lower kinematic profiles of the T2-FIS, using the data filtered by the EKF filter,  represents a more conservative classification. However, the central tendencies of the T2-FIS results using the SavitzkyGolay filter are higher than the K-Means, because the construction of the fuzzy intervals and the rulebase follows a more generic methodology, in contrast to the training of the K-Means algorithm that finds the centers of the clusters that best fit the current dataset. 

% T2-FIS - Random Forest -: $(0.313, 0.218, 0.226, 0.243)$ | $(0.282, 0.275, 0.231, 0.212)$

% The experimental results show that the fuzzy inference system with multiple experts decision-making found lower kinematics profiles and more consistent driving styles classes. The Type-2 Fuzzy Inference System also achieved lower data dispersion in each group, and also lower central tendencies for the \emph{Mean Acceleration} and \emph{Mean Deceleration} kinematics features, in comparison with the Type-1 Fuzzy Inference System. In addition, the T2-FIS also behaves more conservatively than the clustering algorithms, since its driving style classes has lower kinematic profiles for the data filtered with the EKF algorithm, which have the most noise. 
% It is important to highlight that conservative behavior was also adopted in the heuristic for the choice of weights in the OWA method, during the aggregation of the experts' opinions, which reflects in the results of the fuzzy multiple experts systems.


==> tex/tab_clustering.tex <==
\begin{table*}[!bt]
\caption{Clustering - Descriptive Statistics Analysis}
\label{tab:result:clustering:descriptive_stats}

 \resizebox{\textwidth}{!}{
\scriptsize
\centering
\begin{tabular}{cclrrrrrrrrrrrrrrrr}
\hline
\multirow{2}{*}{\textbf{Driving Style}}  & \multirow{2}{*}{\textbf{Filter}}& \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Feature}}} & \multicolumn{4}{c}{\textbf{KMeans}} & \multicolumn{4}{c}{\textbf{GMM Clustering}}   & \multicolumn{4}{c}{\textbf{Fuzzy C-Means}}& \multicolumn{4}{c}{\textbf{Agglomerative Hierarchical Clustering}} \\ \cline{4-19} 
 &   & \multicolumn{1}{c}{}& \multicolumn{1}{c}{\textbf{Mean}} & \multicolumn{1}{c}{\textbf{STD}} & \multicolumn{1}{c}{\textbf{Min}} & \multicolumn{1}{c|}{\textbf{Max}} & \multicolumn{1}{c}{\textbf{Mean}} & \multicolumn{1}{c}{\textbf{STD}} & \multicolumn{1}{c}{\textbf{Min}} & \multicolumn{1}{c|}{\textbf{Max}} & \multicolumn{1}{c}{\textbf{Mean}} & \multicolumn{1}{c}{\textbf{STD}} & \multicolumn{1}{c}{\textbf{Min}} & \multicolumn{1}{c|}{\textbf{Max}} & \multicolumn{1}{c}{\textbf{Mean}} & \multicolumn{1}{c}{\textbf{STD}} & \multicolumn{1}{c}{\textbf{Min}} & \multicolumn{1}{c}{\textbf{Max}} \\ \hline
\multirow{8}{*}{\textbf{Calm}} & \multirow{4}{*}{\textbf{EKF}}   &  \textit{Mean Velocity} ($m/s$) & \textit{8.256}& \textit{4.162}   & 1.285  & \multicolumn{1}{r|}{24.021}   & 8.370   & 4.410  & 1.370  & \multicolumn{1}{r|}{24.021}   & 8.056   & 4.148  & 1.398  & \multicolumn{1}{r|}{24.021}   & 8.484   & 4.177  & 1.285  & 24.021 \\
 &   & \textit{Mean Acceleration} ($m/s^{2}$)  & 4.108   & 1.948  & 0.486  & \multicolumn{1}{r|}{31.374}   & 3.313   & 1.007  & 0.486  & \multicolumn{1}{r|}{5.999}& 3.854   & 1.862  & 0.486  & \multicolumn{1}{r|}{25.735}   & 4.451   & 2.109  & 0.486  & 34.482 \\
 &   & \textit{Mean Deceleration} ($m/s^{2}$)   & 3.910   & 1.815  & 0.373  & \multicolumn{1}{r|}{50.628}   & 3.188   & 0.987  & 0.373  & \multicolumn{1}{r|}{5.923}& 3.664   & 1.734  & 0.373  & \multicolumn{1}{r|}{50.628}   & 4.239   & 1.971  & 0.373  & 50.628 \\
 &   & \textit{STD Lateral Jerk} ($m/s^{3}$)& 36.811  & 15.238 & 1.437  & \multicolumn{1}{r|}{66.028}   & 34.162  & 14.034 & 1.437  & \multicolumn{1}{r|}{75.518}   & 32.635  & 12.562 & 1.437  & \multicolumn{1}{r|}{55.130}   & 42.359  & 19.275 & 1.437  & 84.191 \\ \cline{2-19} 
 & \multirow{4}{*}{\textbf{SavitzkyGolay}} &  \textit{Mean Velocity} ($m/s$) & 5.217   & 1.500  & 1.119  & \multicolumn{1}{r|}{8.092}& 5.829   & 2.117  & 1.144  & \multicolumn{1}{r|}{12.852}   & 4.911   & 1.356  & 1.119  & \multicolumn{1}{r|}{7.457}& 6.487   & 2.269  & 1.119  & 14.432 \\
 &   & \textit{Mean Acceleration} ($m/s^{2}$)  & \textit{1.395}& 0.946  & 0.000  & \multicolumn{1}{r|}{9.761}& 1.553   & 0.736  & 0.000  & \multicolumn{1}{r|}{3.951}& 1.389   & 0.935  & 0.000  & \multicolumn{1}{r|}{9.761}& 1.425   & 0.997  & 0.000  & 12.782 \\
 &   & \textit{Mean Deceleration} ($m/s^{2}$)  & \textit{1.391}& 1.011  & 0.000  & \multicolumn{1}{r|}{12.082}   & 1.510   & 0.750  & 0.000  & \multicolumn{1}{r|}{3.923}& 1.377   & 0.984  & 0.000  & \multicolumn{1}{r|}{11.058}   & 1.422   & 1.043  & 0.000  & 11.422 \\
 &   & \textit{STD Lateral Jerk} ($m/s^{3}$)   & \textit{1.325}& 1.211  & 0.037  & \multicolumn{1}{r|}{15.216}   & 0.986   & 0.559  & 0.037  & \multicolumn{1}{r|}{2.800}& 1.301   & 1.183  & 0.037  & \multicolumn{1}{r|}{14.720}   & 1.459   & 1.241  & 0.033  & 13.772 \\ \hline
\multirow{8}{*}{\textbf{Moderate}}   & \multirow{4}{*}{\textbf{EKF}}   &  \textit{Mean Velocity} ($m/s$) & \textit{10.539}   & 4.100  & 1.437  & \multicolumn{1}{r|}{24.760}   & 9.501   & 4.081  & 1.285  & \multicolumn{1}{r|}{23.050}   & 10.143  & 4.085  & 1.285  & \multicolumn{1}{r|}{24.760}   & 10.890  & 4.098  & 1.437  & 24.760 \\
 &   & \textit{Mean Acceleration} ($m/s^{2}$)  & \textit{7.987}& 2.569  & 1.182  & \multicolumn{1}{r|}{34.482}   & 6.589   & 1.830  & 1.588  & \multicolumn{1}{r|}{12.069}   & 7.069   & 2.339  & 1.182  & \multicolumn{1}{r|}{34.482}   & 8.717   & 2.502  & 1.182  & 24.540 \\
 &   & \textit{Mean Deceleration} ($m/s^{2}$)  & \textit{7.710}& 2.544  & 2.233  & \multicolumn{1}{r|}{34.482}   & 6.229   & 1.748  & 1.381  & \multicolumn{1}{r|}{10.986}   & 6.817   & 2.289  & 2.168  & \multicolumn{1}{r|}{24.760}   & 8.453   & 2.520  & 2.250  & 24.772 \\
 &   & \textit{STD Lateral Jerk} ($m/s^{3}$)   & \textit{98.842}   & 23.254 & 65.056 & \multicolumn{1}{r|}{150.668}  & 75.457  & 30.741 & 2.795  & \multicolumn{1}{r|}{164.630}  & 84.410  & 20.390 & 53.868 & \multicolumn{1}{r|}{127.332}  & 110.511 & 19.554 & 78.929 & 155.889\\ \cline{2-19} 
 & \multirow{4}{*}{\textbf{SavitzkyGolay}} &  \textit{Mean Velocity} ($m/s$) & \textit{10.256}   & 1.565  & 7.472  & \multicolumn{1}{r|}{13.590}   & 11.145  & 3.992  & 1.119  & \multicolumn{1}{r|}{23.983}   & 9.256   & 1.317  & 6.901  & \multicolumn{1}{r|}{11.567}   & 11.412  & 1.121  & 8.726  & 13.989 \\
 &   & \textit{Mean Acceleration} ($m/s^{2}$)  & \textit{1.082}& \textit{0.919}   & 0.000  & \multicolumn{1}{r|}{11.373}   & 0.748   & 0.441  & 0.000  & \multicolumn{1}{r|}{2.352}& 1.182   & 0.986  & 0.000  & \multicolumn{1}{r|}{11.373}   & 0.707   & 0.456  & 0.000  & 3.899  \\
 &   & \textit{Mean Deceleration} ($m/s^{2}$)  & \textit{1.108}& \textit{0.990}   & 0.000  & \multicolumn{1}{r|}{13.420}   & 0.737   & 0.451  & 0.000  & \multicolumn{1}{r|}{2.324}& 1.209   & 1.075  & 0.000  & \multicolumn{1}{r|}{15.031}   & 0.724   & 0.497  & 0.000  & 3.433  \\
 &   & \textit{STD Lateral Jerk} ($m/s^{3}$)   & \textit{1.356}& \textit{1.129}   & 0.033  & \multicolumn{1}{r|}{11.349}   & 1.075   & 0.678  & 0.033  & \multicolumn{1}{r|}{3.568}& 1.394   & 1.225  & 0.033  & \multicolumn{1}{r|}{15.216}   & 0.969   & 0.641  & 0.046  & 3.814  \\ \hline
\multicolumn{1}{l}{\multirow{8}{*}{\textbf{Aggressive}}} & \multirow{4}{*}{\textbf{EKF}}   &  \textit{Mean Velocity} ($m/s$) & \textit{11.537}   & \textit{4.098}   & 1.880  & \multicolumn{1}{r|}{22.959}   & 11.077  & 4.077  & 1.880  & \multicolumn{1}{r|}{24.760}   & 11.496  & 4.135  & 1.880  & \multicolumn{1}{r|}{22.959}   & 11.529  & 4.062  & 1.880  & 22.959 \\
\multicolumn{1}{l}{}   &   & \textit{Mean Acceleration} ($m/s^{2}$)  & \textit{13.908}   & \textit{4.493}   & 2.669  & \multicolumn{1}{r|}{38.759}   & 12.410  & 4.171  & 1.182  & \multicolumn{1}{r|}{38.759}   & 12.663  & 4.266  & 2.253  & \multicolumn{1}{r|}{38.759}   & 14.044  & 4.507  & 2.669  & 38.759 \\
\multicolumn{1}{l}{}   &   & \textit{Mean Deceleration} ($m/s^{2}$)  & \textit{12.743}   & \textit{3.965}   & 2.307  & \multicolumn{1}{r|}{35.312}   & 11.784  & 3.566  & 2.307  & \multicolumn{1}{r|}{50.628}   & 11.777  & 3.797  & 2.307  & \multicolumn{1}{r|}{35.312}   & 12.818  & 3.992  & 2.307  & 35.312 \\
\multicolumn{1}{l}{}   &   & \textit{STD Lateral Jerk} ($m/s^{3}$)   & \textit{203.352}  & \textit{56.289}  & 149.873& \multicolumn{1}{r|}{983.533}  & 154.555 & 69.107 & 4.441  & \multicolumn{1}{r|}{983.533}  & 179.674 & 55.019 & 126.581& \multicolumn{1}{r|}{983.533}  & 205.515 & 56.440 & 149.215& 983.533\\ \cline{2-19} 
\multicolumn{1}{l}{}   & \multirow{4}{*}{\textbf{SavitzkyGolay}} &  \textit{Mean Velocity} ($m/s$) & \textit{15.752}   & \textit{1.693}   & 9.139  & \multicolumn{1}{r|}{33.766}   & 10.740  & 4.519  & 1.249  & \multicolumn{1}{r|}{33.766}   & 14.713  & 2.355  & 10.179 & \multicolumn{1}{r|}{33.766}   & 15.740  & 2.140  & 6.837  & 33.766 \\
\multicolumn{1}{l}{}   &   & \textit{Mean Acceleration} ($m/s^{2}$)  & \textit{1.175}& \textit{1.336}   & 0.000  & \multicolumn{1}{r|}{19.074}   & 2.493   & 1.734  & 0.000  & \multicolumn{1}{r|}{19.074}   & 1.095   & 1.188  & 0.000  & \multicolumn{1}{r|}{19.074}   & 1.204   & 1.362  & 0.000  & 19.074 \\
\multicolumn{1}{l}{}   &   & \textit{Mean Deceleration} ($m/s^{2}$)  & \textit{1.272}& 1.461  & 0.000  & \multicolumn{1}{r|}{21.951}   & 2.826   & 1.787  & 0.000  & \multicolumn{1}{r|}{21.951}   & 1.174   & 1.299  & 0.000  & \multicolumn{1}{r|}{21.951}   & 1.334   & 1.542  & 0.000  & 21.951 \\
\multicolumn{1}{l}{}   &   & \textit{STD Lateral Jerk} ($m/s^{3}$)   & \textit{1.693}& 1.791  & 0.096  & \multicolumn{1}{r|}{26.908}   & 3.590   & 2.098  & 0.065  & \multicolumn{1}{r|}{26.908}   & 1.572   & 1.587  & 0.064  & \multicolumn{1}{r|}{26.908}   & 1.762   & 1.873  & 0.096  & 26.908 \\ \hline
\end{tabular}
}

\end{table*}


==> tex/tab_distances.tex <==
\begin{table*}[!bt]
    \caption{Interquartile Ranges of T1-FIS and T2-FIS}
    \label{tab:distance_kmeans_fuzzy}
     \resizebox{\textwidth}{!}{
 \scriptsize
 \centering
 \begin{tabular}{llcrrrrr}
\cline{3-8}
\multicolumn{2}{l}{\multirow{3}{*}{}}    & \multicolumn{3}{c}{\textbf{EKF}}         & \multicolumn{3}{c}{\textbf{SavitzkyGolay}}      \\ \cline{3-8} 
\multicolumn{2}{l}{}    & \multicolumn{6}{c}{\textbf{K-Means}}             \\ \cline{3-8} 
\multicolumn{2}{l}{}    & \textit{calm}             & \multicolumn{1}{c}{\textit{moderate}} & \multicolumn{1}{c|}{\textit{aggressive}} & \multicolumn{1}{c}{\textit{calm}} & \multicolumn{1}{c}{\textit{moderate}} & \multicolumn{1}{c}{\textit{aggressive}} \\ \cline{3-8} 
\multicolumn{1}{c}{\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}T2-FIS \\ \\ (Multiple)\end{tabular}}}} & calm              & \multicolumn{1}{r}{28.08} & \textit{89.41}       & \multicolumn{1}{r|}{197.62}              & \textit{1.72}    & 3.46                 & \textit{9.16}          \\
\multicolumn{1}{c}{} & \textit{moderate} & \multicolumn{1}{r}{9.65}  & 71.01                & \multicolumn{1}{r|}{179.29}              & 7.77             & 2.72                 & 3.08  \\
\multicolumn{1}{c}{} & aggressive        & \multicolumn{1}{r}{49.89} & 11.61                & \multicolumn{1}{r|}{119.91}              & 17.91            & 11.44                & 7.66  \\ \hline
\end{tabular}
    }
\end{table*}

==> tex/tab_fuzzy.tex <==
\begin{table*}[!bt]
    \caption{Fuzzy Inference System - Descriptive Statistics Analysis}
    \label{tab:fuzzy_result}
     \resizebox{\textwidth}{!}{
        \scriptsize
        \centering
\begin{tabular}{cclrrrrrrrrrrrrrrrr}
\hline
\multirow{2}{*}{\textbf{Driving Style}}                  & \multirow{2}{*}{\textbf{Filter}}        & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Feature}}} & \multicolumn{4}{c}{\textbf{T1-FIS (Single)}}                                    & \multicolumn{4}{c}{\textbf{T1-FIS (Multiple)}}                                  & \multicolumn{4}{c}{\textbf{T2-FIS (Single)}}                                    & \multicolumn{4}{c}{\textbf{T2-FIS (Multiple)}}                                 \\ \cline{4-19} 
                                                         &                                         & \multicolumn{1}{c}{}                                  & \multicolumn{1}{c}{\textbf{Mean}} & \multicolumn{1}{c}{\textbf{STD}} & \multicolumn{1}{c}{\textbf{Min}} & \multicolumn{1}{c|}{\textbf{Max}} & \multicolumn{1}{c}{\textbf{Mean}} & \multicolumn{1}{c}{\textbf{STD}} & \multicolumn{1}{c}{\textbf{Min}} & \multicolumn{1}{c|}{\textbf{Max}} & \multicolumn{1}{c}{\textbf{Mean}} & \multicolumn{1}{c}{\textbf{STD}} & \multicolumn{1}{c}{\textbf{Min}} & \multicolumn{1}{c|}{\textbf{Max}} & \multicolumn{1}{c}{\textbf{Mean}} & \multicolumn{1}{c}{\textbf{STD}} & \multicolumn{1}{c}{\textbf{Min}} & \multicolumn{1}{c}{\textbf{Max}} \\ \hline
\multirow{8}{*}{\textbf{Calm}}                           & \multirow{4}{*}{\textbf{EKF}}           & \textit{Mean Velocity} ($m/s$)                                & \textit{4.606}                    & \textit{1.702}                   & 1.861                            & \multicolumn{1}{r|}{9.860}        & 3.513                             & 0.941                            & 1.861                            & \multicolumn{1}{r|}{8.374}        & 4.802                             & 2.133                            & 1.861                            & \multicolumn{1}{r|}{10.790}       & 3.556                             & 0.950                            & 1.861                            & 8.374                            \\
                                                         &                                         & \textit{Mean Acceleration} ($m/s^{2}$)                                     & 1.798                             & 0.685                            & 0.486                            & \multicolumn{1}{r|}{5.474}        & 1.737                             & 0.640                            & 0.518                            & \multicolumn{1}{r|}{3.270}        & 1.551                             & 0.483                            & 0.486                            & \multicolumn{1}{r|}{2.996}        & 1.565                             & 0.511                            & 0.486                            & 2.996                            \\
                                                         &                                         & \textit{Mean Deceleration} ($m/s^{2}$)                                     & 1.709                             & 0.597                            & 0.373                            & \multicolumn{1}{r|}{3.694}        & 1.642                             & 0.581                            & 0.373                            & \multicolumn{1}{r|}{3.269}        & 1.502                             & 0.443                            & 0.373                            & \multicolumn{1}{r|}{2.876}        & 1.499                             & 0.457                            & 0.373                            & 2.537                            \\
                                                         &                                         & \textit{STD Lateral Jerk} ($m/s^{3}$)                                      & 7.497                             & 2.201                            & 1.437                            & \multicolumn{1}{r|}{10.549}       & 7.157                             & 2.377                            & 1.437                            & \multicolumn{1}{r|}{10.524}       & 7.777                             & 2.322                            & 1.437                            & \multicolumn{1}{r|}{10.999}       & 7.464                             & 2.450                            & 1.437                            & 10.999                           \\ \cline{2-19} 
                                                         & \multirow{4}{*}{\textbf{SavitzkyGolay}} & \textit{Mean Velocity} ($m/s$)                                & 8.164                             & 3.222                            & 1.119                            & \multicolumn{1}{r|}{14.285}       & 5.713                             & 1.799                            & 1.119                            & \multicolumn{1}{r|}{8.729}        & 8.830                             & 3.706                            & 1.119                            & \multicolumn{1}{r|}{16.354}       & 6.673                             & 2.413                            & 1.119                            & 10.799                           \\
                                                         &                                         & \textit{Mean Acceleration} ($m/s^{2}$)                            & \textit{1.136}                    & 0.784                            & 0.000                            & \multicolumn{1}{r|}{6.257}        & 1.237                             & 0.749                            & 0.000                            & \multicolumn{1}{r|}{6.257}        & 1.060                             & 0.726                            & 0.000                            & \multicolumn{1}{r|}{5.877}        & 1.086                             & 0.665                            & 0.000                            & 5.877                            \\
                                                         &                                         & \textit{Mean Deceleration} ($m/s^{2}$)                            & \textit{1.133}                    & 0.808                            & 0.000                            & \multicolumn{1}{r|}{6.193}        & 1.203                             & 0.743                            & 0.000                            & \multicolumn{1}{r|}{5.988}        & 1.056                             & 0.751                            & 0.000                            & \multicolumn{1}{r|}{6.003}        & 1.059                             & 0.659                            & 0.000                            & 5.988                            \\
                                                         &                                         & \textit{STD Lateral Jerk} ($m/s^{3}$)                             & \textit{1.237}                    & 0.924                            & 0.033                            & \multicolumn{1}{r|}{9.974}        & 1.165                             & 0.861                            & 0.037                            & \multicolumn{1}{r|}{9.974}        & 1.173                             & 0.835                            & 0.033                            & \multicolumn{1}{r|}{7.897}        & 1.116                             & 0.794                            & 0.033                            & 6.996                            \\ \hline
\multirow{8}{*}{\textbf{Moderate}}                       & \multirow{4}{*}{\textbf{EKF}}           & \textit{Mean Velocity} ($m/s$)                                & \textit{6.798}                    & 2.695                            & 1.479                            & \multicolumn{1}{r|}{14.949}       & 6.752                             & 3.004                            & 1.479                            & \multicolumn{1}{r|}{14.949}       & 7.520                             & 2.795                            & 1.544                            & \multicolumn{1}{r|}{17.750}       & 7.008                             & 3.425                            & 1.544                            & 17.750                           \\
                                                         &                                         & \textit{Mean Acceleration} ($m/s^{2}$)                            & \textit{3.672}                    & 1.314                            & 0.627                            & \multicolumn{1}{r|}{8.168}        & 3.075                             & 0.984                            & 0.486                            & \multicolumn{1}{r|}{8.168}        & 3.713                             & 1.311                            & 0.709                            & \multicolumn{1}{r|}{8.168}        & 2.697                             & 0.858                            & 0.627                            & 8.168                            \\
                                                         &                                         & \textit{Mean Deceleration} ($m/s^{2}$)                            & \textit{3.391}                    & 1.210                            & 0.644                            & \multicolumn{1}{r|}{7.609}        & 2.829                             & 0.793                            & 0.644                            & \multicolumn{1}{r|}{7.609}        & 3.475                             & 1.269                            & 0.702                            & \multicolumn{1}{r|}{8.359}        & 2.473                             & 0.689                            & 0.644                            & 6.811                            \\
                                                         &                                         & \textit{STD Lateral Jerk} ($m/s^{3}$)                             & \textit{37.698}                   & 20.161                           & 3.643                            & \multicolumn{1}{r|}{192.741}      & 30.350                            & 13.789                           & 2.795                            & \multicolumn{1}{r|}{142.778}      & 38.910                            & 20.962                           & 2.795                            & \multicolumn{1}{r|}{192.741}      & 25.660                            & 11.402                           & 2.696                            & 168.585                          \\ \cline{2-19} 
                                                         & \multirow{4}{*}{\textbf{SavitzkyGolay}} & \textit{Mean Velocity} ($m/s$)                                & \textit{15.107}                   & 3.282                            & 1.916                            & \multicolumn{1}{r|}{33.766}       & 12.463                            & 3.082                            & 1.916                            & \multicolumn{1}{r|}{20.539}       & 13.788                            & 4.712                            & 1.441                            & \multicolumn{1}{r|}{25.899}       & 12.813                            & 3.524                            & 1.441                            & 22.916                           \\
                                                         &                                         & \textit{Mean Acceleration} ($m/s^{2}$)                            & \textit{1.357}                    & \textit{1.346}                   & 0.000                            & \multicolumn{1}{r|}{12.782}       & 1.140                             & 1.038                            & 0.000                            & \multicolumn{1}{r|}{12.782}       & 1.873                             & 1.528                            & 0.000                            & \multicolumn{1}{r|}{19.074}       & 1.287                             & 1.138                            & 0.000                            & 11.373                           \\
                                                         &                                         & \textit{Mean Deceleration} ($m/s^{2}$)                            & \textit{1.493}                    & \textit{1.526}                   & 0.000                            & \multicolumn{1}{r|}{13.698}       & 1.219                             & 1.167                            & 0.000                            & \multicolumn{1}{r|}{13.698}       & 2.082                             & 1.677                            & 0.000                            & \multicolumn{1}{r|}{13.698}       & 1.385                             & 1.277                            & 0.000                            & 13.698                           \\
                                                         &                                         & \textit{STD Lateral Jerk} ($m/s^{3}$)                             & \textit{1.855}                    & \textit{1.730}                   & 0.101                            & \multicolumn{1}{r|}{11.615}       & 1.520                             & 1.322                            & 0.033                            & \multicolumn{1}{r|}{15.216}       & 2.465                             & 1.966                            & 0.065                            & \multicolumn{1}{r|}{13.966}       & 1.650                             & 1.429                            & 0.046                            & 15.216                           \\ \hline
\multicolumn{1}{l}{\multirow{8}{*}{\textbf{Aggressive}}} & \multirow{4}{*}{\textbf{EKF}}           & \textit{Mean Velocity} ($m/s$)                                & \textit{11.002}                   & \textit{4.344}                   & 1.285                            & \multicolumn{1}{r|}{24.760}       & 10.436                            & 4.303                            & 1.285                            & \multicolumn{1}{r|}{24.760}       & 10.483                            & 4.660                            & 1.285                            & \multicolumn{1}{r|}{24.760}       & 9.923                             & 4.307                            & 1.285                            & 24.760                           \\
\multicolumn{1}{l}{}                                     &                                         & \textit{Mean Acceleration} ($m/s^{2}$)                            & \textit{8.062}                    & \textit{4.018}                   & 1.182                            & \multicolumn{1}{r|}{38.759}       & 7.683                             & 3.853                            & 1.182                            & \multicolumn{1}{r|}{38.759}       & 7.949                             & 4.052                            & 1.182                            & \multicolumn{1}{r|}{38.759}       & 7.204                             & 3.837                            & 1.182                            & 38.759                           \\
\multicolumn{1}{l}{}                                     &                                         & \textit{Mean Deceleration} ($m/s^{2}$)                            & \textit{7.723}                    & \textit{3.620}                   & 1.500                            & \multicolumn{1}{r|}{50.628}       & 7.339                             & 3.507                            & 1.500                            & \multicolumn{1}{r|}{50.628}       & 7.586                             & 3.680                            & 1.554                            & \multicolumn{1}{r|}{50.628}       & 6.867                             & 3.520                            & 1.554                            & 50.628                           \\
\multicolumn{1}{l}{}                                     &                                         & \textit{STD Lateral Jerk} ($m/s^{3}$)                             & \textit{96.489}                   & \textit{58.982}                  & 5.999                            & \multicolumn{1}{r|}{983.533}      & 91.106                            & 57.001                           & 5.999                            & \multicolumn{1}{r|}{983.533}      & 94.507                            & 59.614                           & 5.414                            & \multicolumn{1}{r|}{983.533}      & 84.703                            & 56.245                           & 5.414                            & 983.533                          \\ \cline{2-19} 
\multicolumn{1}{l}{}                                     & \multirow{4}{*}{\textbf{SavitzkyGolay}} & \textit{Mean Velocity} ($m/s$)                                & \textit{16.903}                   & \textit{4.084}                   & 4.113                            & \multicolumn{1}{r|}{31.314}       & 18.159                            & 4.796                            & 4.392                            & \multicolumn{1}{r|}{33.766}       & 17.718                            & 4.645                            & 4.113                            & \multicolumn{1}{r|}{33.766}       & 17.037                            & 5.393                            & 5.118                            & 33.766                           \\
\multicolumn{1}{l}{}                                     &                                         & \textit{Mean Acceleration} ($m/s^{2}$)                            & \textit{4.587}                    & \textit{3.176}                   & 0.315                            & \multicolumn{1}{r|}{19.074}       & 4.330                             & 3.339                            & 0.203                            & \multicolumn{1}{r|}{19.074}       & 4.781                             & 3.189                            & 0.417                            & \multicolumn{1}{r|}{17.386}       & 5.810                             & 3.117                            & 0.492                            & 19.074                           \\
\multicolumn{1}{l}{}                                     &                                         & \textit{Mean Deceleration} ($m/s^{2}$)                            & \textit{5.113}                    & 3.020                            & 0.000                            & \multicolumn{1}{r|}{21.951}       & 4.428                             & 3.551                            & 0.000                            & \multicolumn{1}{r|}{21.951}       & 5.084                             & 3.237                            & 0.000                            & \multicolumn{1}{r|}{21.951}       & 5.691                             & 3.450                            & 0.000                            & 21.951                           \\
\multicolumn{1}{l}{}                                     &                                         & \textit{STD Lateral Jerk} ($m/s^{3}$)                             & \textit{6.595}                    & 3.921                            & 0.388                            & \multicolumn{1}{r|}{26.908}       & 5.947                             & 4.417                            & 0.117                            & \multicolumn{1}{r|}{26.908}       & 6.652                             & 4.173                            & 0.507                            & \multicolumn{1}{r|}{26.908}       & 7.748                             & 4.009                            & 0.551                            & 26.908                           \\ \hline
\end{tabular}
    }
\end{table*}

